Distributed Training of Embeddings using Graph Analytics

Many applications today, such as NLP, network analysis, and code analysis, rely on semantically embedding objects into low-dimensional fixed-length vectors. Such embeddings naturally provide a way to perform useful downstream tasks, such as identifying relations among objects or predicting objects for a given context, etc. Unfortunately, the training necessary for accurate embeddings is usually computationally intensive and requires processing large amounts of data. Furthermore, distributing this training is challenging. Most embedding training uses stochastic gradient descent (SGD), an "inherently" sequential algorithm. Prior approaches to parallelizing SGD do not honor these dependencies and thus potentially suffer poor convergence. This paper presents a distributed training framework for a class of applications that use Skip-gram-like models to generate embeddings. We call this class Any2Vec and it includes Word2Vec, DeepWalk, and Node2Vec among others. We first formulate Any2Vec training algorithm as a graph application and leverage the state-of-the-art distributed graph analytics framework, D-Galois. We adapt D-Galois to support dynamic graph generation and repartitioning, and incorporate novel communication optimizations. Finally, we introduce a novel way to combine gradients during distributed training to prevent accuracy loss. We show that our framework, called GraphAny2Vec, matches on a cluster of 32 hosts the accuracy of the state-of-the-art shared-memory implementations of Word2Vec and Vertex2Vec on 1 host, and gives a geo-mean speedup of 12x and 5x respectively. Furthermore, GraphAny2Vec is on average 2x faster than the state-of-the-art distributed Word2Vec implementation, DMTK, on 32 hosts. We also show the superiority of our Gradient Combiner independent of GraphAny2Vec by incorporating it in DMTK, which raises its accuracy by > 30%.

==> tbl_3rdparty.tex <==
% \begin{table}[t]
% \footnotesize
% \caption{Execution time (sec) of \wordtovec and Gensim on 1 host and \graphwordvec on 32 hosts, 
% and speedup of \graphwordvec over \wordtovecend.}
% \label{tbl:3rdparty_time}
%  \centering
\begin{tabular}{@{ }l@{\hskip1.8pt}|r@{\hskip5pt}|r@{\hskip5pt}|r@{\hskip5pt}|r@{\hskip5pt}|r@{\hskip5pt}|r@{\hskip5pt}|r@{\hskip3pt}r@{\hskip5pt}r@{ }}
  \toprule
  \multicolumn{1}{c|}{\textbf{Dataset}}         & \multicolumn{1}{c|}{\textbf{W2V}} & \multicolumn{1}{c|}{\textbf{GEM}} & \multicolumn{1}{c|}{\textbf{GW2V}} & \multicolumn{1}{c|}{\textbf{Speedup}} \\ 
\midrule 
\multirow{1}{*}{\textbf{1-billion}} & 22957.9               & 17516.1                & 1633.5                  & 14.0x                          \\ 
\multirow{1}{*}{\textbf{news}}      & 25278.2              & 19376.8              & 1731.1                  & 14.6x                        \\
\multirow{1}{*}{\textbf{wiki}}     & 140216.8              &  OOM                        & 9993.7                  & 14.0x                          \\ 

  \bottomrule
\end{tabular}
%\end{table}


==> tbl_3rdparty_accuracy.tex <==
\begin{table*}[t]
\footnotesize
\centering
%\caption{3rd Party comparisons: Accuracy}
  \caption{Accuracy (semantic, syntactic, and total) of \wordtovec and Gensim on 1 host and \graphwordvec on 32 hosts.}
\label{tbl:3rdparty_acc}
%\begin{tabular}{|l|l|l|l|l|l|l|l|l|l|}
\begin{tabular}{@{ }l@{\hskip1.8pt}|r@{\hskip5pt}r@{\hskip5pt}r@{\hskip5pt}r@{\hskip5pt}r@{\hskip5pt}r@{\hskip5pt}r@{\hskip3pt}r@{\hskip5pt}r@{ }}
  \toprule
  \multicolumn{1}{c|}{\textbf{Dataset}}         & \multicolumn{3}{c|}{Semantic} & \multicolumn{3}{|c|}{Syntactic} & \multicolumn{3}{|c}{Total} \\ 
  \cline{2-10}
          & \multicolumn{1}{c}{W2V}      &\multicolumn{1}{c}{GEN}      & \multicolumn{1}{c|}{GW2V}    &\multicolumn{1}{|c}{W2V}      & \multicolumn{1}{c}{GEN}      &\multicolumn{1}{c|}{GW2V}     &\multicolumn{1}{|c}{W2V}     & \multicolumn{1}{c}{GEN}     & \multicolumn{1}{c}{GW2V}   \\ 
  \midrule
  \multirow{1}{*}{\textbf{1-billion}} & 75.93    & 75.93    &  \multicolumn{1}{c|}{74.79}   &  \multicolumn{1}{|c}{51}       & 50.56    &  \multicolumn{1}{c|}{48.78}    &  \multicolumn{1}{|c}{72.36}   & 72.36   & 71.64  \\ 
  \multirow{1}{*}{\textbf{news}}      & 70.79    & 70.57    & \multicolumn{1}{c|}{68.86}   & \multicolumn{1}{|c}{50.2}     & 50.52    & \multicolumn{1}{c|}{50.11}    & \multicolumn{1}{|c}{69.21}   & 69.07   & 67.79   \\ 
  \multirow{1}{*}{\textbf{wiki}}      & 79.1     &          & \multicolumn{1}{c|}{77.93}   & \multicolumn{1}{|c}{49.22}    &          & \multicolumn{1}{c|}{48.4}     & \multicolumn{1}{|c}{74.1}    &         & 73.43  \\ 
  \bottomrule
\end{tabular}
\end{table*}



==> tbl_3rdparty_accuracy_long.tex <==
\begin{table}[t]
  \footnotesize
  \centering
  \caption{Accuracy (semantic, syntactic, and total) of \wordtovec and Gensim on 1 host and \graphwordvec on 32 hosts.}
  \label{tbl:3rdparty_acc}
    \begin{tabular}{@{ }l@{\hskip1.8pt}|r@{\hskip5pt}r@{\hskip5pt}r@{\hskip5pt}r@{ }}
      \toprule
       & \multicolumn{1}{c|}{\textbf{Dataset}}         & \multicolumn{1}{c|}{\textbf{1-billion}} & \multicolumn{1}{|c|}{\textbf{news}} & \multicolumn{1}{|c}{\textbf{wiki}} \\ 
      \midrule
      \multirow{3}{*}{\textbf{Semantic}} & \multicolumn{1}{c|}{W2V}  & \multicolumn{1}{c|}{75.93}    & \multicolumn{1}{c|}{70.79}    &  \multicolumn{1}{c}{79.10} \\
                                         &\multicolumn{1}{c|}{GEN}  & \multicolumn{1}{c|}{75.93}    &\multicolumn{1}{c|}{70.57}    &  \multicolumn{1}{c}{} \\
                                         %\rowcolor{green!20}
&\multicolumn{1}{c|}{\colorbox{green!20}{{GW2V}}} & \multicolumn{1}{c|}{\colorbox{white!20}{76.07}}    &\multicolumn{1}{c|}{\colorbox{white!20}{70.86}}    &  \multicolumn{1}{c}{\colorbox{white!20}{78.93}} \\

      \midrule
      \multirow{3}{*}{\textbf{Syntactic}} & \multicolumn{1}{c|}{W2V}  & \multicolumn{1}{c|}{51.00}    & \multicolumn{1}{c|}{50.2}    &  \multicolumn{1}{c}{49.22} \\
                                         &\multicolumn{1}{c|}{GEN}  & \multicolumn{1}{c|}{50.56}    &\multicolumn{1}{c|}{50.52}    &  \multicolumn{1}{c}{} \\
                                         %\rowcolor{green!20}
                   &\multicolumn{1}{c|}{\colorbox{green!20}{{GW2V}}} & \multicolumn{1}{c|}{\colorbox{white!20}{50.10}}    &\multicolumn{1}{c|}{\colorbox{white!20}{50.11}}    &  \multicolumn{1}{c}{\colorbox{white!20}{48.40}} \\

      \midrule
      \multirow{3}{*}{\textbf{Total}} & \multicolumn{1}{c|}{W2V}  & \multicolumn{1}{c|}{72.36}    & \multicolumn{1}{c|}{69.21}    &  \multicolumn{1}{c}{74.10} \\
                                         &\multicolumn{1}{c|}{GEN}  & \multicolumn{1}{c|}{72.36}    &\multicolumn{1}{c|}{69.07}    &  \multicolumn{1}{c}{} \\
                                         %\rowcolor{green!20}
                   &\multicolumn{1}{c|}{\colorbox{green!20}{{GW2V}}} & \multicolumn{1}{c|}{\colorbox{white!20}{72.50}}    &\multicolumn{1}{c|}{\colorbox{white!20}{69.50}}    &  \multicolumn{1}{c}{\colorbox{white!20}{73.93}} \\


     \bottomrule
    \end{tabular}
  \end{table}



==> tbl_all_accuracy_long.tex <==
\begin{table}[t]
   \footnotesize
  \centering
  \caption{Accuracy (semantic, syntactic, and total) of \wordtovec and Gensim on 1 host and \graphwordvec on 32 hosts.}
  \label{tbl:3rdparty_acc}
    \begin{tabular}{@{ }l@{\hskip1.8pt}|r@{\hskip5pt}r@{\hskip5pt}r@{\hskip5pt}r@{ }}
      \toprule
       & \multicolumn{1}{c|}{\textbf{Dataset}}         & \multicolumn{1}{c|}{\textbf{1-billion}} & \multicolumn{1}{|c|}{\textbf{news}} & \multicolumn{1}{|c}{\textbf{wiki}} \\ 
      \midrule
      \multirow{8}{*}{\rotatebox[origin=c]{90}{\textbf{Semantic}}} & \multicolumn{1}{l|}{\colorbox{white!20}{W2V}}  & \multicolumn{1}{c|}{75.86 }    & \multicolumn{1}{c|}{70.79 }    &  \multicolumn{1}{c}{79.10 } \\
                                         &\multicolumn{1}{l|}{\colorbox{white!20}{GEN}} & \multicolumn{1}{c|}{75.64 }    &\multicolumn{1}{c|}{70.57 }    &  \multicolumn{1}{c}{OOM} \\
                                         %\rowcolor{green!20}
                                         &\multicolumn{1}{l|}{\colorbox{white!20}{DMTL(AVG) (1 Host)}} & \multicolumn{1}{c|}{\colorbox{white!20}{62.07 }} &\multicolumn{1}{c|}{\colorbox{white!20}{52.36}}    &  \multicolumn{1}{c}{\colorbox{white!20}{71.64 }} \\
                                         &\multicolumn{1}{l|}{\colorbox{white!20}{DMTL(AVG) (32 Host)}} & \multicolumn{1}{c|}{\colorbox{white!20}{18.50 }}    &\multicolumn{1}{c|}{\colorbox{white!20}{13.64 }}    &  \multicolumn{1}{c}{\colorbox{white!20}{44.71 }} \\

                                         &\multicolumn{1}{l|}{\colorbox{white!20}{DMTL(GP) (1 Host)}} & \multicolumn{1}{c|}{\colorbox{white!20}{62.07 }}    &\multicolumn{1}{c|}{\colorbox{white!20}{52.36}}    &  \multicolumn{1}{c}{\colorbox{white!20}{71.64 }} \\
                                         &\multicolumn{1}{l|}{\colorbox{white!20}{DMTL(GP) (32 Host)}} & \multicolumn{1}{c|}{\colorbox{white!20}{64.93 }}    &\multicolumn{1}{c|}{\colorbox{white!20}{53.79 }}    &  \multicolumn{1}{c}{\colorbox{white!20}{73.93 }} \\

                                         &\multicolumn{1}{l|}{\colorbox{green!20}{{GW2V(AVG) (1 Host)}}} & \multicolumn{1}{c|}{\colorbox{white!20}{75.93 }}    &\multicolumn{1}{c|}{\colorbox{white!20}{70.71 }}    &  \multicolumn{1}{c}{\colorbox{white!20}{79.36 }} \\
                                         &\multicolumn{1}{l|}{\colorbox{green!20}{{GW2V(AVG) (32 Host)}}} & \multicolumn{1}{c|}{\colorbox{white!20}{68.86 }}    &\multicolumn{1}{c|}{\colorbox{white!20}{61.64 }}    &  \multicolumn{1}{c}{\colorbox{white!20}{75.07 }} \\


                                         &\multicolumn{1}{l|}{\colorbox{green!20}{{GW2V(GP) (1 Host)}}} & \multicolumn{1}{c|}{\colorbox{white!20}{75.79 }}    &\multicolumn{1}{c|}{\colorbox{white!20}{70.10 }}    &  \multicolumn{1}{c}{\colorbox{white!20}{79.2 }} \\
                                         &\multicolumn{1}{l|}{\colorbox{green!20}{{GW2V(GP) (32 Host)}}} & \multicolumn{1}{c|}{\colorbox{white!20}{76.07 }}    &\multicolumn{1}{c|}{\colorbox{white!20}{70.86 }}    &  \multicolumn{1}{c}{\colorbox{white!20}{78.93 }} \\

      \midrule
      \multirow{8}{*}{\rotatebox[origin=c]{90}{\textbf{Syntactic}}} & \multicolumn{1}{l|}{\colorbox{white!20}{W2V}}  & \multicolumn{1}{c|}{50.00  }    & \multicolumn{1}{c|}{50.0 }    &  \multicolumn{1}{c}{49.22 } \\
                                         &\multicolumn{1}{l|}{\colorbox{white!20}{GEN}}  & \multicolumn{1}{c|}{49.86 }    &\multicolumn{1}{c|}{49.88 }    &  \multicolumn{1}{c}{OOM} \\

                                         &\multicolumn{1}{l|}{\colorbox{white!20}{DMTL(AVG) (1 Host)}} & \multicolumn{1}{c|}{48.11 }&  \multicolumn{1}{c|}{49.33 }& \multicolumn{1}{c}{46.11 }\\ 
                                         &\multicolumn{1}{l|}{\colorbox{white!20}{DMTL(AVG) (32 Host)}} & \multicolumn{1}{c|}{25.11 }&\multicolumn{1}{c|}{24.89 }&\multicolumn{1}{c}{26.11 }\\

                                         &\multicolumn{1}{l|}{\colorbox{white!20}{DMTL(GP) (1 Host)}} &\multicolumn{1}{c|}{48.21 } &\multicolumn{1}{c|}{49.33}&\multicolumn{1}{c}{46.11 }\\
                                         &\multicolumn{1}{l|}{\colorbox{white!20}{DMTL(GP) (32 Host)}} &\multicolumn{1}{c|}{46.44 }&\multicolumn{1}{c|}{48.22 }&\multicolumn{1}{c}{47.78 }\\

                                         &\multicolumn{1}{l|}{\colorbox{green!20}{{GW2V(AVG) (1 Host)}}} & \multicolumn{1}{c|}{\colorbox{white!20}{49.21  }}    &\multicolumn{1}{c|}{\colorbox{white!20}{49.67 }}    &  \multicolumn{1}{c}{\colorbox{white!20}{49.22 }} \\
                                         &\multicolumn{1}{l|}{\colorbox{green!20}{{GW2V(AVG) (32 Host)}}} & \multicolumn{1}{c|}{\colorbox{white!20}{45.11 }}    &\multicolumn{1}{c|}{\colorbox{white!20}{45.89 }}    &  \multicolumn{1}{c}{\colorbox{white!20}{41.67 }} \\

                                         %\rowcolor{green!20}
                                         &\multicolumn{1}{l|}{\colorbox{green!20}{{GW2V(GP) (1 Host)}}} & \multicolumn{1}{c|}{\colorbox{white!20}{49.63 }}    &\multicolumn{1}{c|}{\colorbox{white!20}{50.00 }}    &  \multicolumn{1}{c}{\colorbox{white!20}{49.10 }} \\
                                         &\multicolumn{1}{l|}{\colorbox{green!20}{{GW2V(GP) (32 Hosts)}}} & \multicolumn{1}{c|}{\colorbox{white!20}{50.10 }}    &\multicolumn{1}{c|}{\colorbox{white!20}{50.11 }}    &  \multicolumn{1}{c}{\colorbox{white!20}{49.40 }} \\

      \midrule
      \multirow{8}{*}{\rotatebox[origin=c]{90}{\textbf{Total}}} & \multicolumn{1}{l|}{\colorbox{white!20}{W2V}}  & \multicolumn{1}{c|}{72.36 }    & \multicolumn{1}{c|}{69.21 }    &  \multicolumn{1}{c}{74.10 } \\
                                         &\multicolumn{1}{l|}{\colorbox{white!20}{GEN}}  & \multicolumn{1}{c|}{72.36 }    &\multicolumn{1}{c|}{69.07  }    &  \multicolumn{1}{c}{OOM} \\



                                         &\multicolumn{1}{l|}{\colorbox{white!20}{DMTL(AVG) (1 Host)}} & \multicolumn{1}{c|}{60.71 }& \multicolumn{1}{c|}{53.79 }& \multicolumn{1}{c}{71.07 }\\ 
                                         &\multicolumn{1}{l|}{\colorbox{white!20}{DMTL(AVG) (32 Host)}}&\multicolumn{1}{c|}{21.07 }& \multicolumn{1}{c|}{17.50 }& \multicolumn{1}{c}{42.07 }\\

                                         &\multicolumn{1}{l|}{\colorbox{white!20}{DMTL(GP) (1 Host)}} &\multicolumn{1}{c|}{60.71 }&\multicolumn{1}{c|}{53.79 }&\multicolumn{1}{c}{71.07 }\\
                                         &\multicolumn{1}{l|}{\colorbox{white!20}{DMTL(GP) (32 Host)}} &\multicolumn{1}{c|}{62.50 }&\multicolumn{1}{c|}{54.43 }&\multicolumn{1}{c}{68.86 }\\

                                         &\multicolumn{1}{l|}{\colorbox{green!20}{{GW2V(AVG) (1 Host)}}} & \multicolumn{1}{c|}{\colorbox{white!20}{72.14 }}    &\multicolumn{1}{c|}{\colorbox{white!20}{68.79 }}    &  \multicolumn{1}{c}{\colorbox{white!20}{74.20 }} \\
                                         &\multicolumn{1}{l|}{\colorbox{green!20}{{GW2V(AVG) (32 Host)}}} & \multicolumn{1}{c|}{\colorbox{white!20}{65.57  }}    &\multicolumn{1}{c|}{\colorbox{white!20}{59.93 }}    &  \multicolumn{1}{c}{\colorbox{white!20}{68.93 }} \\

                                         %\rowcolor{green!20}
                                         &\multicolumn{1}{l|}{\colorbox{green!20}{{GW2V(GP) (1 Host)}}} & \multicolumn{1}{c|}{\colorbox{white!20}{72.22 }}    &\multicolumn{1}{c|}{\colorbox{white!20}{68.93 }}    &  \multicolumn{1}{c}{\colorbox{white!20}{74.20 }} \\
                                         &\multicolumn{1}{l|}{\colorbox{green!20}{{GW2V(GP) (32 Hosts)}}} & \multicolumn{1}{c|}{\colorbox{white!20}{72.50  }}    &\multicolumn{1}{c|}{\colorbox{white!20}{69.50 }}    &  \multicolumn{1}{c}{\colorbox{white!20}{73.93 }} \\


     \bottomrule
    \end{tabular}
  \end{table}



==> tbl_dmlt_accuracy.tex <==
\begin{table}[t]
\footnotesize
\centering
% \caption{3rd Party comparisons: Accuracy}
\caption{Accuracy (semantic, syntactic, and total) of DMTK~\protect\cite{DMTK} on 32 hosts with Average reduction (AVG) Vs. 
  Model combiner (MC).}
\label{tbl:dmtk_avg_mc}
%\begin{tabular}{|l|l|l|l|l|l|l|l|l|l|}
\begin{tabular}{@{ }l@{\hskip1.8pt}|r@{\hskip5pt}r@{\hskip5pt}r@{\hskip5pt}r@{\hskip5pt}r@{\hskip5pt}r@{\hskip5pt}r@{\hskip3pt}r@{\hskip5pt}r@{ }}
  \toprule
  \multicolumn{1}{c|}{\textbf{Dataset}}         & \multicolumn{2}{c|}{\textbf{Semantic}} & \multicolumn{2}{c}{\textbf{Syntactic}} & \multicolumn{2}{|c}{\textbf{Total}} \\ 
  \cline{2-7}
          & \multicolumn{1}{c}{\textbf{AVG}}      &\multicolumn{1}{c}{\textbf{MC}}    &\multicolumn{1}{|c}{\textbf{AVG}}      & \multicolumn{1}{c}{\textbf{MC}}     &\multicolumn{1}{|c}{\textbf{AVG}}     & \multicolumn{1}{c}{\textbf{MC}}   \\ 
  \midrule
  \multirow{1}{*}{\textbf{1-billion}} &  41.07      & \multicolumn{1}{c}{\colorbox{green!20}{70.07}}   &  \multicolumn{1}{|c}{42.44}         &  \multicolumn{1}{c|}{\colorbox{green!20}{48.67}}    &  \multicolumn{1}{c}{43.14}    & \colorbox{green!20}{68.14}  \\ 
  \multirow{1}{*}{\textbf{news}}      &  30.29       & \multicolumn{1}{c|}{\colorbox{green!20}{62.93}}   & \multicolumn{1}{|c}{42.89}       & \multicolumn{1}{c|}{\colorbox{green!20}{49.78}}    & \multicolumn{1}{|c}{35.07}    &  \colorbox{green!20}{62.57}  \\ 
  % \multirow{1}{*}{\textbf{wiki}}      &          & \multicolumn{1}{c|}{}   & \multicolumn{1}{|c}{}      & \multicolumn{1}{c|}{}     & \multicolumn{1}{|c}{}     &   \\ 
  \bottomrule
\end{tabular}
\end{table}

==> tbl_dmtk_gw2v.tex <==
 \begin{table}[t]
 \footnotesize
 \caption{Execution time (sec) of \wordtovec in DMTK Vs \graphwordvec,
 and speedup of \graphwordvec over DMTK's \wordtovec on 32 hosts on 1-billion and news text datasets.}
 \label{tbl:dmtk_time}
  \centering
\begin{tabular}{@{ }l@{\hskip1.8pt}|r@{\hskip5pt}|r@{\hskip5pt}|r@{\hskip5pt}|r@{\hskip5pt}|r@{\hskip5pt}|r@{\hskip3pt}r@{\hskip5pt}r@{ }}
%\begin{tabular}{lllll}
  \toprule
  \multicolumn{1}{c|}{\textbf{Dataset}}         & \multicolumn{1}{c|}{\textbf{DMTK}} &  \multicolumn{1}{c|}{\textbf{GW2V}} & \multicolumn{1}{c|}{\textbf{Speedup}} \\ 
\midrule 
\multirow{1}{*}{\textbf{1-billion}} & 2175.72               & 1160.93                &    1.9x                               \\ 
\multirow{1}{*}{\textbf{news}}      & 2556.92              & 1336.08              &       1.9x                                \\

  \bottomrule
\end{tabular}
\end{table}


==> tbl_node2vec_acc_small.tex <==
\begin{table*}[t]
    \footnotesize
    \centering
    %\caption{3rd Party comparisons: Accuracy}
      \caption{Accuracy (Macro F1 and Micro F1) of \wordtovec and Deepwalk on 1 host and \graphwordvec on ?? hosts.}
    \label{tbl:3rdparty_acc}
    %\begin{tabular}{|l|l|l|l|l|l|l|l|l|l|}
      \begin{tabular}{@{ }l@{\hskip1.8pt}|r@{\hskip5pt}r@{\hskip5pt}r@{\hskip5pt}r@{\hskip5pt}r@{\hskip5pt}r@{\hskip5pt}r@{\hskip3pt}r@{\hskip5pt}}
      \toprule
      \multicolumn{1}{c|}{\textbf{Dataset}}         & \multicolumn{2}{c|}{BlogCatalog} & \multicolumn{2}{|c|}{Flickr} & \multicolumn{2}{|c}{Youtube} \\ 
      %\multicolumn{1}{c|}{\textbf{\% Labeled Nodes}}         & \multicolumn{1}{c|}{10\%} & \multicolumn{1}{|c|}{20\%} & \multicolumn{1}{|c}{10\%} \\ 
      \cline{2-7}
                            & \multicolumn{1}{c}{Macro-F1}      &\multicolumn{1}{c}{Micro-F1}          &\multicolumn{1}{|c}{Macro-F1}      & \multicolumn{1}{c}{Micro-F1}      &\multicolumn{1}{|c}{Macro-F1}     & \multicolumn{1}{c}{Micro-F1}  \\ 
      \midrule
      \multirow{1}{*}{\textbf{Deepwalk}} & 75.93       &  \multicolumn{1}{c|}{74.79}   &  \multicolumn{1}{|c}{51}         &  \multicolumn{1}{c|}{48.78}    &  \multicolumn{1}{|c}{72.36}   & 72.36  \\ 
      \multirow{1}{*}{\textbf{GW2V}}      & 70.79       & \multicolumn{1}{c|}{68.86}   & \multicolumn{1}{|c}{50.2}         & \multicolumn{1}{c|}{50.11}    & \multicolumn{1}{|c}{69.21}     & 69.07    \\ 
      \bottomrule
    \end{tabular}
    \end{table*}
    
    


==> tbl_time_all.tex <==
\begin{table*}[t]
\footnotesize
\caption{Execution time (sec) of all.}
\label{tbl:all_time}
 \centering
%\begin{tabular}{@{ }l@{\hskip1.8pt}|r@{\hskip5pt}|r@{\hskip5pt}|r@{\hskip5pt}|r@{\hskip5pt}|r@{\hskip5pt}|r@{\hskip5pt}|r@{\hskip3pt}r@{\hskip5pt}r@{\hskip5pt}r@{ }}
\begin{tabular}{l|r|r|r|r|r|r|r|r|r|r}

    \toprule
    \multicolumn{1}{c|}{\textbf{Dataset}}   & \multicolumn{1}{c|}{\textbf{W2V}} & \multicolumn{1}{c|}{\textbf{GEM}} & \multicolumn{2}{c|}{\textbf{DMTL(AVG)}}& \multicolumn{2}{c|}{\textbf{DMTL(GP)}}& \multicolumn{2}{c|}{\textbf{GW2V(AVG)}} & \multicolumn{2}{c|}{\textbf{GW2V(GP)}} \\ 
  \midrule
     & \multicolumn{1}{c|}{\textbf{1 Hosts}} & \multicolumn{1}{c|}{\textbf{1 Host}} &  \multicolumn{1}{c|}{\textbf{1 Host}} & \multicolumn{1}{c|}{\textbf{32 Hosts}}&  \multicolumn{1}{c|}{\textbf{1 Host}}&\multicolumn{1}{c|}{\textbf{32 Host}} & \multicolumn{1}{c|}{\textbf{1 Hosts}}  & \multicolumn{1}{c|}{\textbf{32 Hosts}}&\multicolumn{1}{c|}{\textbf{1 Host}} & \multicolumn{1}{c|}{\textbf{32 Hosts}} \\ 
  \midrule 
  \multirow{1}{*}{\textbf{1-billion}} &   15261.3     &  15828.2   & 15156.9 &2081.0        &15136.9      & 2175.7         & 14679.9& 1129.1    &  14334.0                 &  1160.9              \\ 
  \multirow{1}{*}{\textbf{news}}      &   16037.8     &  16782.8   & 15438.6   & 2571.0       &  15288.3   & 2556.9           &15998.1 & 1360.6   &  16254.7                 &1336.1              \\
  \multirow{1}{*}{\textbf{wiki}}      &   73757.6      &  OOM       & 91562.1   & 12081.2       & 91562.1  &  12041.1         &80470.6  &  6846.2  &  80437.3                 &  6647.5      \\ 
  
    \bottomrule
  \end{tabular}
  \end{table*}
  

